A Survey on Offensive AI Within Cybersecurity

Artificial Intelligence (AI) has witnessed major growth and integration across various domains. As AI systems become increasingly prevalent, they also become targets for threat actors to manipulate their functionality for malicious purposes. This survey paper on offensive AI will comprehensively cover various aspects related to attacks against and using AI systems. It will delve into the impact of offensive AI practices on different domains, including consumer, enterprise, and public digital infrastructure. The paper will explore adversarial machine learning, attacks against AI models, infrastructure, and interfaces, along with offensive techniques like information gathering, social engineering, and weaponized AI. Additionally, it will discuss the consequences and implications of offensive AI, presenting case studies, insights, and avenues for further research.

==> listings/ART_sklearn_full.tex <==
"""
The script demonstrates a simple example of using ART with scikit-learn. The example train a small model on the MNIST
dataset and creates adversarial examples using the Fast Gradient Sign Method. Here we use the ART classifier to train
the model, it would also be possible to provide a pretrained model to the ART classifier.
The parameters are chosen for reduced computational requirements of the script and not optimised for accuracy.
"""
from sklearn.svm import SVC
import numpy as np

from art.attacks.evasion import FastGradientMethod
from art.estimators.classification import SklearnClassifier
from art.utils import load_mnist

# Step 1: Load the MNIST dataset

(x_train, y_train), (x_test, y_test), min_pixel_value, max_pixel_value = load_mnist()

# Step 1a: Flatten dataset

nb_samples_train = x_train.shape[0]
nb_samples_test = x_test.shape[0]
x_train = x_train.reshape((nb_samples_train, 28 * 28))
x_test = x_test.reshape((nb_samples_test, 28 * 28))

# Step 2: Create the model

model = SVC(C=1.0, kernel="rbf")

# Step 3: Create the ART classifier

classifier = SklearnClassifier(model=model, clip_values=(min_pixel_value, max_pixel_value))

# Step 4: Train the ART classifier

classifier.fit(x_train, y_train)

# Step 5: Evaluate the ART classifier on benign test examples

predictions = classifier.predict(x_test)
accuracy = np.sum(np.argmax(predictions, axis=1) == np.argmax(y_test, axis=1)) / len(y_test)
print("Accuracy on benign test examples: {}%".format(accuracy * 100))

# Step 6: Generate adversarial test examples
attack = FastGradientMethod(estimator=classifier, eps=0.2)
x_test_adv = attack.generate(x=x_test)

# Step 7: Evaluate the ART classifier on adversarial test examples

predictions = classifier.predict(x_test_adv)
accuracy = np.sum(np.argmax(predictions, axis=1) == np.argmax(y_test, axis=1)) / len(y_test)
print("Accuracy on adversarial test examples: {}%".format(accuracy * 100))
